MAVBench: Micro Aerial Vehicle Benchmarking

Unmanned Aerial Vehicles (UAVs) are getting closer to becoming ubiquitous in everyday life. Among them, Micro Aerial Vehicles (MAVs) have seen an outburst of attention recently, specifically in the area with a demand for autonomy. A key challenge standing in the way of making MAVs autonomous is that researchers lack the comprehensive understanding of how performance, power, and computational bottlenecks affect MAV applications. MAVs must operate under a stringent power budget, which severely limits their flight endurance time. As such, there is a need for new tools, benchmarks, and methodologies to foster the systematic development of autonomous MAVs. In this paper, we introduce the `MAVBench' framework which consists of a closed-loop simulator and an end-to-end application benchmark suite. A closed-loop simulation platform is needed to probe and understand the intra-system (application data flow) and inter-system (system and environment) interactions in MAV applications to pinpoint bottlenecks and identify opportunities for hardware and software co-design and optimization. In addition to the simulator, MAVBench provides a benchmark suite, the first of its kind, consisting of a variety of MAV applications designed to enable computer architects to perform characterization and develop future aerial computing systems. Using our open source, end-to-end experimental platform, we uncover a hidden, and thus far unexpected compute to total system energy relationship in MAVs. Furthermore, we explore the role of compute by presenting three case studies targeting performance, energy and reliability. These studies confirm that an efficient system design can improve MAV's battery consumption by up to 1.8X.

==> tex/analysis.tex <==
\section{Analysis}

In this section we characterize our workloads and determine the components of a drone's subsystem that their performance is most affected by. Thus, we get an accurate picture of exactly what is being tested by each workload.

We see that workload X stresses the parallel processing capability of a drone's companion computer, while workload Y's performance is unaffected by such-and-such component, etc.


==> tex/optimization.tex <==
\section{Context-Sensitive Optimization}
\label{sec:optimization}

As was shown in the previous section, the OctoMap generation node plays a crucial role in performance and energy consumption of drones.
This node is used for modeling of various environment without prior assumptions. In order to do so, the map of the environment is maintained in an efficient tree-like data structure while keeping track of free, occupied and unknown areas. Both planning and collision avoidance kernels utilize this data structure to make safe flights possible by only allowing the drone to navigate through free spaces.  

size of the voxels, i.e. the map's resolution, trades off accuracy and flight-time/energy. By lowering the resolution, i.e. increasing voxel sizes, obstacle boundaries get inflated, hence drones perception of the environment and the objects within it becomes inaccurate. However, doing so improves the performance of the OctoMap generation node and eventually leads to a faster flight time.  As figure blah shows blahx speed up in the update rate of OctoMap is achievable for a sacrifice of blahx in resolution. 

To study the effect of this knob on our applications we conducted a study where the drone will conduct some part of its mission in less dense environment such as outdoors and part of it in more dense environment such as indoors. We 



the  the flight time and the energy consumption of the drone. This node is responsible for providing the 

==> tex/performance.tex <==
\section{Performance Characterization}

% Characterizations of each of our micro- and macro-benchmarks. We describe which drone applications require parallel computer architectures, which ones require computers with fast serial performance, and which ones would benefit from parallel architectures but run fast enough on serial computers.

We plot the performance breakdowns of our micro-benchmarks in Fig~\ref{fig:micro-perf}. We found that computer vision kernels such as \textit{object detection} achieve high performance only on computers with highly parallel  architectures such as the TX1. We found that SLAM micro-benchmarks require such-and-such architecture to achieve high performance. We found that the path-finding micro-benchmarks achieve high performance on all our processors, but they achieve even higher performance on computers with such-and-such architecture.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/micro-perf}
\caption{Performance of computational micro-benchmarks on various companion computers.}
\label{fig:micro-perf}
\end{figure}

We plot the performance breakdowns of our macro-benchmarks when running in simulated environments designed for AirSim, as seen in Fig.~\ref{fig:perf-breakdown}. We find, in general, that computer vision tasks act as our applications' bottlenecks.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/perf-breakdown}
\caption{Performance breakdown of \textit{Person Tracking} benchmark on AirSim with various companion computers.}
\label{fig:perf-breakdown}
\end{figure}


==> tex/power.tex <==
\section{Power Characterization}

We characterized the power consumption of drones when executing simple flight maneuvers as well as when executing macro-benchmarks person-tracking.

As a drone's size increases, its motors become responsible for a larger and larger portion of its power consumption, until the motors consume nearly all the power generated by a drone. Fig.~\ref{fig:power-hover-solo} illustrates the power distribution on a large MAV such as the 3DR Solo, while Fig.~\ref{fig:power-hover-nano} illustrates the power distribution of a much lighter and smaller nano-aerial vehicle such as the Hummingbird.

\begin{figure}[h]
\centering

  \subfloat[Large micro-aerial vehicle.]
  {\includegraphics[width=.9\linewidth]{figs/power-hover-solo}
  \label{fig:power-hover-solo}}

  \subfloat[Small nano-aerial vehicle.]
  {\includegraphics[width=.9\linewidth]{figs/power-hover-nano}
  \label{fig:power-hover-nano}}

\caption{Resolution vs performance on the drone.}
\label{fig:power-distribution}
\end{figure}

Thus, as a drone's size falls, it's flight time increasingly depends upon the power consumed by its companion computer, as well as the power required to lift its computer into the air. In Fig.~\ref{fig:flight-time-tracking-tx1}, we plot the flight time of our drones when executing the \textit{Person Tracking} benchmark. The drones are equipped with a TX1 giving them 20 FPS performance.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/flight-time-tracking-tx1}
\caption{Flight time of drones when executing \textit{Person Tracking} benchmark with TX1.}
\label{fig:flight-time-tracking-tx1}
\end{figure}

In Fig.~\ref{fig:perf-tracking-10min}, on the other hand, we plot the performance of the \textit{Person Tracking} application when running on various drones equipped with the most performant computer that will allow them to achieve 10 minutes of flight time.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/perf-tracking-10min}
\caption{Performance of drones when executing \textit{Person Tracking} benchmark with 10 minutes of flight time.}
\label{fig:perf-tracking-10min}
\end{figure}

In Fig.~\ref{fig:energy-search-and-rescue}, we plot the total energy spent by our simulated AirSim drone when completing the \textit{Search-and-Rescue} macrobenchmark with various companion computers. As more powerful computers are used, our simulated drone is able to fly faster without missing potential targets and is thus able to complete its mission faster with less total energy expenditure.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/energy-search-and-rescue}
\caption{Energy expended by AirSim drone when executing \textit{Person Tracking} benchmark with various companion computers.}
\label{fig:energy-search-and-rescue}
\end{figure}


==> tex/scratch.tex <==
   \section{misc}
   
   \textbf{high lighting our benchmark:}  
   \begin{itemize}
   \item Our first version of MAVBench includes applications from different yet popular Micro Aerial Vehicle’s use cases although this benchmark is not inclusive to all that's out there. 
   
   \item we expect our benchmark to evolove with the help of both communities
   \item though MAV has been a hot topic within the robotic domain for a while and has gained attraction, there has been a lack of attention from the system/architecture domain
   
   
   \end{itemize}
   
   \textbf{highlighting our simulation platform}
   \begin{itemize}
   \item talk about the crash based and how we win.
   \end{itemize}
   
   we should highlight that besides benefits such as cost that is usually the reason behind simulation for systems, safety and reproducibility possibiities provided by simulation is of high importance for aerial agents
   
   in defense of ROS(http://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=6213236) 
   
    //talk about nodelets and the difference they make 
   //talk about gps denied environments
   
   weakpoints of ROS(singl point of failure ie. roscore and not secure) http://www.theconstructsim.com/start-self-driving-cars-using-ros/
  
  
  random thoughts: leads focus (and optimization) of wrong kernels. we have been talking about detection as an example. Remind me to talk to you about localization as well). Note that if we encounter recurring kernels as bottlenecks, we can motivate for design of system with a specialized accelerator capable running multiple applications ,  where as if we see different bottlenecks, we can motivate for design of systems, each of which is good at a specific application
    
    todo:A picture for each applications:
High level pipeline
Think about micro benchmarking (e.g. the effect of intelligence on the energy)
. 
\red{misc: talk about unpredicated events (Taken care in motion controllers). Perception: information about the environment state (e.g object localizations, ...) and the drone itself.}

Tight constraints: their form factor places tight constraints on the amount of possible energy on board (figure blah). Such energy constraints limits the flight time demanding (figure blah) fast and intelligent decision making withing such a limited flight time.


==> tex/software_pipeline.tex <==
High-level software pipeline associated with our (though not exclusive to it) workloads are shown in figure blah. 

\textbf{perception stage:}
Perception is defined as "the task- oriented interpretation of sensor data" ~\cite{Handbook_robotic}. Inputs to this stage, the sensory data (e.g. GPS) and a partial model of the environment (voxel map), are fused to develop a more elaborate model (e.g. improved voxel map) in order to extract the drone's and environment's relevant states (e.g. position of obstacles around the drone). 

\textbf{Planning:}
Using the inputs (e.g. voxel map) from the perception stage, the next two steps (namely planning and control) provide a motion generation framework \footnote{Our benchmark suit solely focuses on motion planning}. Planning involves generating (usually) a \textit{collision-free} to a target. In a nutshell, this step involves first generating a set of possible paths to the target (e.g. PRM) and then choosing an optimal one among them using a a path-planning algorithm (e.g. A*). 


\textbf{Control:}
This stage is about achieving a desired path (provided from the previous stage) while providing a set of guarantees such as feasibility, stability and robustness~\cite{tech_problem}. In this stage, drones dynamics are considered and flight commands are generated while ensuring the aforementioned guarantees.  


==> tex/suite.tex <==
\section{Benchmarking Suite}



Our benchmarking suite tests the performance of drones when executing a diverse set of tasks that are either commonly executed by drones today or that are being vigorously researched.

Our benchmarking suite is made of various workloads that are split into two categories: micro-benchmarks and macro-benchmarks. Micro-benchmarks test the capability of a drone to execute a single, very narrow task that may be used as a kernel in many other, larger applications. Macro-benchmarks test the capability of a drone to execute a complete mission, such as delivering a package or searching for and rescuing a person in need.

Our benchmarking suite records the speed with which a drone is able to complete a task, and the power it consumes in doing so, as well as certain measures that are specific to the workload being run.

\subsection{Micro-benchmarks}

\subsection{Macro-benchmarks}


==> tex/sys-arch.tex <==
\section{System Architecture} % Maybe change to "simulation architecture"

\begin{comment}
\begin{figure}[t]
\centering
\includegraphics[width=6cm, height=4cm ,keepaspectratio]{figs/robot_arch.png}
\caption{System architecture of a typical robotic agent.}
\end{figure}
\end{comment}
%In this section, we provide an architectural overview of typical drone platforms in order to provide the background necessary to understand their architectural constraints, and the requirements for a simulator that can provide insights into those constraints.

% \textcolor{red}{Like any other robotic systems, drones have 3 subsystems: ....}
%\subsection{Accuracy Impact:}
\begin{figure}[t!]
\centering
\includegraphics[width=0.9\columnwidth]{figs/agent_env.pdf}
\vspace{1.0ex}
\caption{Agent-environment model.}
\vspace{-3ex}
\label{fig:1}
\end{figure}
Given the aforementioned constrains, these agents demand architects attention. In this section, we provide the architectural overview of such agents as the first step toward a design around such constrains.  

Like other robotic agents, such systems operate by sampling the environment state, interpreting and reacting to it using three main subsystems, namely, a sensory subsystem, a perception subsystem, and an actuation subsystem. Fig.~\ref{} shows these subsystems and their corresponding data and energy flow. More concretely, Fig.~\ref{} shows the details of each subsystem \textcolor{red}{(have various sensors and actuator names on the figure.)}
\begin{comment}
\begin{figure}
\includegraphics[width=6cm, height=4cm ,keepaspectratio]{figs/drone_arch.png}
\caption{Detailed system architecture of an aerial robotic agent.}
\end{figure}
\end{comment}
\begin{comment}
Sensor subsystem: is usually comprised of a versatile set of sensors such as cameras, IMU (inertial measurement units), IR, lidar, etc depending on size, energy budget and other constraints.
Perception subsystem: This system is responsible for processing the sampled data. typical off-the-shelf UAVs, such as the 3DR Solo, are equipped with at least two on-board processors: a ``companion computer'' that handles workloads, and a ``flight controller'' responsible for high to low (and vice versa) conversion of sensing and actuation subcommands (e.g. conversion of hover (high level) command to specific rotor speed (low level)).
Actuation subsystem: this system is responsible for reacting and modifying the world around the agent. It ranges anywhere from rather simple rotors to robotic arms capable of grasping and lifting objects. 
}


\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/drone-architecture}
\caption{Architectural overview of a typical drone platform. \textcolor{red}{Iterate over this figure; it should be improved.}}
\label{fig:dronearch}
\end{figure}
\end{comment}

\textbf{Sensory Subsystem} To enable intelligent flight, drones must be equipped with a rich set of sensors that are capable of gathering visual, depth, position, and orientation data. For example, to detect possible intruders and separate them from authorized visitors, an autonomous security drone will require image data from cameras. To detect the positions of obstacles, a drone would also require depth information from stereo or RGBD cameras. Number and type of sensors is highly dependent on the workload requirement such as, and various system constraints such as perception subsystem capability to process them. 

\textbf{Perception Subsystem} To enable intelligent flight, drones must also come equipped with on-board companion computers that are capable of performing high-level cognitive \textcolor{red}{(this probably isn't the right word here)} tasks, such as object classification and obstacle avoidance. Such processors must satisfy various constraints such as drone's thermal and energy limit,form factor, etc. Therefore, many off-the-shelf drone platforms such as the Solo come equipped with small, low-power processors such as the ARM Cortex-M A9 that struggle to provide real-time cognitive capability for compute-heavy tasks such as visual classification. For higher performance, UAV designers can turn to other state-of-the-art embedded systems such as the NVIDIA TX2, although these systems incur higher power penalties. In addition to the companion computers, typically, drone platforms come with a ``flight controller'' responsible for high to low (and vice versa) conversion of sensing and actuation subcommands (e.g. conversion of hover (high level) command to specific rotor speed (low level).

\textbf{Actuation Subsystem} This system is responsible for reacting and modifying the world around the agent. It ranges anywhere from rather simple rotors to robotic arms capable of grasping and lifting objects.
Similar to sensors, their type and number is highly a function of the workload and processing power on board. 


==> tex/todos.tex <==
1. be consistent across applications for collecting the maximum allowed velocity
2. run more experiments per applications
3. what element of compute matters (improve on the heat map) and draw conclusions about whether concurrency and so on matters?
4. integrate slam. 
5. table is not clear.

6. related work include an optimization works (such as slam and knobs) 
7. related work: the duke paper (the start up)
8. cite Jason Clemons http://www.eecs.umich.edu/eecs/about/articles/2012/Clemons-NVIDIA.html


